Period Adaptation for Continuous Security Monitoring in Multicore Real-Time Systems

We propose a design-time framework (named HYDRA-C) for integrating security tasks into partitioned real-time systems (RTS) running on multicore platforms. Our goal is to opportunistically execute security monitoring mechanisms in a 'continuous' manner -- i.e., as often as possible, across cores, to ensure that security tasks run with as few interruptions as possible. Our framework will allow designers to integrate security mechanisms without perturbing existing real-time (RT) task properties or execution order. We demonstrate the framework using a proof-of-concept implementation with intrusion detection mechanisms as security tasks. We develop and use both, (a) a custom intrusion detection system (IDS), as well as (b) Tripwire -- an open source data integrity checking tool. These are implemented on a realistic rover platform designed using an ARM multicore chip. We compare the performance of HYDRA-C with a state-of-the-art RT security integration approach for multicore-based RTS and find that our method can, on average, detect intrusions 19.05% faster without impacting the performance of RT tasks.

==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

LATEX = pdflatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> Review_comments/dac19link.tex <==
https://docs.google.com/document/d/1SwcpUD9QDaADjPzk1DtjTrVXWsK4MDHbJ3eFgIardnQ/edit?usp=sharing

==> Sections/intro_old.tex <==
\section{Introduction}
\label{sec:intro}

% \hl{Whole Section is Revised -- MH}

% \hl{NOTE: Can you please assist me to improve and expand abstract/intro to better motivate the problem? We have some space to fill -- MH}

Limited resources in terms of processing power, memory, energy, \etc~coupled with the fact that security was not considered a design priority has led to the deployment of a large number of real-time systems (RTS) that include little to no security mechanisms. Hence, retrofitting such legacy RTS with general-purpose security solutions is a challenging problem since any perturbation of the real-time (RT) constraints
(runtimes, periods, task execution orders, deadlines, \etc) could be detrimental
to the correct and safe operation of RTS. 
%Security solutions that are  proposed for traditional Integrating security mechanisms for legacy systems is not an easy tasks since these mechanisms must \textit{co-exist} with the existing real-time (RT) tasks in the system. 
Besides, security mechanisms need to be designed in such a way that an adversary can not easily evade them. Successful attacks/intrusions into
RTS are often aimed at impacting the safety guarantees of such systems, as evidenced by 
%The concern about real-time systems (RTS) security is growing and the breaches are not uncommon on safety-critical systems as evident by 
recent intrusions (\eg attacks on control systems~\cite{stuxnet, Ukraine16}, automobiles~\cite{ris_rts_1, checkoway2011comprehensive}, medical devices~\cite{security_medical}, \etc~to name but a few).
%Any successful attack can result in the safety of such systems being
%compromised, leading to disastrous effects from damages to the critical infrastructure and environment as well as loss of human life. 
Systems with RT properties pose unique security challenges -- these systems are required to meet stringent timing requirements along with strong safety requirements. 
Limited resources (\ie
computational power, storage, energy, \etc) prevent security mechanisms that have been primarily developed for general purpose
systems from being effective for RTS. 
%It is not straightforward to develop a security solution for the legacy systems, \ie the exiting RT systems where the perturbation of existing constraints for constituent tasks (such as run-times, period, task execution order, \etc) is not allowed/feasible. This is because, any security mechanism has to \ca co-exist with the existing real-time (RT) tasks in the system and \cb operate without impacting the timing and safety constraints.
%\todo[inline]{adding some bridge text}

% Developing a security solution for the legacy systems -- (\ie the exiting RT systems where the perturbation of  constraints such as run-times, period, task execution order, \etc for the existing tasks is not allowed/feasible) -- is not an easy tasks. 


% It is not straightforward to develop a security solution for the legacy systems, \ie the exiting RT systems where the perturbation of existing constraints for constituent tasks (such as run-times, period, task execution order, \etc) is not allowed/feasible. This is because, any security mechanism has to \ca co-exist with the existing real-time (RT) tasks in the system and \cb operate without impacting the timing and safety constraints.

\todo[inline]{RBB: Bring For instance., consider an IDS ... text here}

\todo[inline]{RBB: As a step towards enabling the design of secure RT platforms researchers proposed Opportunistic execution ...}

Opportunistic execution~\cite{mhasan_rtss16,mhasan_date18} has been proposed as a potential way to integrate security mechanisms into legacy RTS --  this allows the execution of security mechanisms as background services without impacting the timing constraints of the RT tasks. Other approaches have been built on this technique for integrating tasks into both legacy and non-legacy systems~\cite{mhasan_ecrts17,xie2007improving,lin2009static,lesi2017network,lesi2017security,securecore,hamad2018prediction}. However, most of that work was focused on single core RTS (that are a majority of such systems in use today). However, \textit{multicore} processors have found increased use in the design of RTS to improve overall performance and energy efficiency~\cite{rt_multicore_lui,mutiprocessor_survey}. 
While the use of such processors \textit{increases} the security problems in RTS (\eg due to parallel execution of critical tasks)~\cite{mhasan_rtiot_sensors19} very few security solutions have been proposed in literature. 

\todo[inline]{RBB: In this paper we propose ....}


In early work (called \prefname)~\cite{mhasan_date18} researchers have developed some mechanisms for integrating security into multicore RTS -- however this work does not allow runtime migration of security tasks across cores and \hl{we show that this} may result in delayed detection of intrusions\footnote{We discuss this issue further in  Section~\ref{sec:evaluation}.}.

%that may result in a delayed detection of intrusions\footnote{We discuss this issue further in  Section~\ref{sec:evaluation}.}.

% uses a very restricted system model especially for the security tasks (\ie security tasks can not migrate across cores at runtime and that may result in a delayed detection of an intrusion). %\todo{what are the restrictions?}



%\todo[inline]{RBB: Looks like we are restarting here after talking about HYDRA}
As a step towards the design of secure RT platforms, we propose
to improve the security posture of a multicore-based RTS through integration of security tasks. Our main goal in this paper is \textit{to raise the responsiveness of such security tasks by increasing their frequency of execution}. For instance, consider an intrusion detection system (IDS) -- say one that checks the integrity of file systems. If such a system is interrupted (before it can complete checking the entire system), then an adversary could use that opportunity to intrude into the system and, perhaps, stay resident in the part of the filesystem that has already been checked (assuming that the IDS is carrying out the check in parts). If, on the other hand, the IDS task is able to execute with as few interruptions as possible (\textit{e.g.}, by moving immediately to an empty core when it is interrupted), then there is much higher chance of success and, correspondingly, a much lower chance of a successful adversarial action.
Note that the addition of any security mechanisms (such as IDS, encryption/authentication, behavior-based monitoring, \etc) may require modification of the system or the RT task parameters as was the case in prior work~\cite{xie2007improving,lin2009static,lesi2017network,lesi2017security, securecore,securecore_memory,securecore_syscal,xie2005dynamic,sibin_RT_security_journal}. %In this paper we focus on situations where addition of security mechanisms do not require any system-level modifications. 
Our focus is on
ensuring that the existing RT tasks are not affected by such integration. The security tasks could be carrying out any one of protection, detection or response-based operations, depending on the system requirements. For instance, a sensor measurement correlation task may be added for detecting sensor manipulation or a change detection task (or other intrusion detection programs) may be added to detect changes/intrusions into the system. 


% \begin{note*}
	 \note
	 We do not target our framework towards any specific security mechanism -- our focus is to integrate any designer-provided security solution into a multicore-based RTS.
% \end{note*}
In Table \ref{tab:mc_se_ex_table} we present some examples of security tasks that can be integrated into legacy systems (again, this is by no stretch meant to be an exhaustive list). In our experiments we used Tripwire~\cite{tripwire} (a data integrity checking tool) as well as our \textit{in-house custom-developed malicious kernel module checker} to demonstrate the feasibility of our approach -- the ideas proposed in this paper are more broadly applicable \hl{to other security mechanisms}.








\begin{table}[!thb]
% \renewcommand{\arraystretch}{1.3}
\caption{Example of Security Tasks}
\label{tab:mc_se_ex_table}
\centering
\hspace*{-0.5em}
\begin{tabular}{P{3.65cm}||P{4.2cm}}
\hline %\\
\bfseries Security Task & \bfseries Approach/Tools\\
\hline\hline
File-system checking & Tripwire~\cite{tripwire}, AIDE~\cite{aide}, \etc \\
Network packet monitoring & Bro~\cite{bro}, Snort~\cite{snort}, \etc \\
Hardware event monitoring & Statistical analysis based checks~\cite{woo2018early} using performance monitors (\eg \text{perf}~\cite{linux_perf}, \texttt{OProfile}~\cite{oprofile}, \etc)\\ 
Application specific checking & Behavior-based detection (see the related work~\cite{anomaly_detection_survey, securecore,securecore_memory,securecore_syscal}) \\
\hline
\end{tabular}
\end{table}




% RTS have also been moving towards the use of {\em multicore} 
%processors due to higher performance and better energy efficiency. In this research our goal is to \textit{improve the security posture of a multicore-based RT platform by integrating security tasks without violating timing constraints}. The security tasks could be any one of protection, detection or response mechanisms, depending on the system requirements. For instance a sensor measurement correlation task may be added for detecting sensor manipulation or a change detection task may be added to detect changes/intrusions into the system. The security tasks can also used for monitoring system behaviors (such as the execution time~\cite{slack_cornell,securecore}, memory access pattern~\cite{securecore_memory}, system call usage~\cite{securecore_syscal}) and/or encryption of communication messages~\cite{xie2007improving,lin2009static,lesi2017network,lesi2017security}. The addition of such tasks may require architectural modifications~\cite{securecore,securecore_memory,securecore_syscal, slack_cornell,mhasan_resecure_iccps} or necessitate changing the schedule or parameters of real-time tasks~\cite{xie2007improving,lin2009static, sibin_RT_security_journal,lesi2017network,lesi2017security}. 
%In contrast, we focus on situations where added security tasks are not allowed to impact the schedule of existing RT tasks when integrating security mechanisms in the system. We highlight that we do not model any specific intrusion detection mechanisms -- our focus here is on the \textit{integration of any designer provided security solutions} for the legacy multicore platform.




\paragraph*{Our Contributions}
In this paper, we propose a design-time methodology and a framework named \pnamemcex for partitioned\footnote{Since this is the commonly used multicore scheduling approach for many commercial and open-source OSs (such as OKL4~\cite{okl4}, QNX~\cite{qnx}, RT-Linux~\cite{rt_patch}, \etc) -- mainly due to its simplicity and efficiency~\cite{parti_see,mhasan_date18}.} RTS that \ci allows security tasks to execute \emph{continuously} (\ie execute as frequently as possible) across cores (\eg follow a \textit{semi-partitioned}~\cite{kato2009semi} RT scheduling scheme); and \cii does not impact the timing constraints of other, existing, RT tasks. Our framework takes advantage of the properties of a multicore platform and allows security tasks to migrate across available cores and execute \textit{opportunistically} (\ie when the RT tasks are not running). This framework extends \hl{existing} work~\cite{mhasan_date18} and ensures better security (\eg faster detection time) and schedulability (see Section \ref{sec:evaluation}). As in previous work~\cite{mhasan_rtss16,mhasan_ecrts17,mhasan_date18} we propose to integrate security mechanisms as independent periodic tasks. To provide the best protection, \textit{security tasks may need to be executed as often as possible}. If the interval between consecutive monitoring events is too large then an attacker may remain undetected and cause harm to the system between two invocations of the security task. In contrast, if the security tasks are executed very frequently, it may impact the schedulability of the RT (and other security) tasks. The challenge is then to determining the right \textit{periods} (\ie minimum inter-invocation time) for the security tasks~\cite{sibin_deeply}. We therefore develop an iterative algorithm that finds the trade-off between schedulability and periods of the security tasks (Section \ref{sec:alg}). 

% In this paper we have the following contributions:

% \begin{enumerate}
% \item A security integration framework, \pnamemcex, for legacy multicore platforms that \textit{allows security tasks to execute continuously} across cores. \pnamemcex is able to do this without violating timing constraints for either the existing RT tasks or the security ones (Section \ref{sec:se_int_frmakework}).

% \item A mathematical model and iterative solution that allows security tasks to execute as frequently as possible while still considering the schedulability constraints of other tasks (Section \ref{sec:period_selection}).
% \end{enumerate}

\todo[inline]{RBB: seem somewhat repetitive. Monwar I would like to chat about flow of Inro. }
A major contribution of this paper is to introduce a security integration framework, \pnamemcex, for legacy multicore platforms that \textit{allows security tasks to execute continuously} across cores. \pnamemcex is able to do this without violating timing constraints for either the existing RT tasks or the security ones (Section \ref{sec:se_int_frmakework}). We develop a mathematical model and iterative solution that allows security tasks to execute as frequently as possible while still considering the schedulability constraints of other tasks (Section \ref{sec:period_selection}). In addition, we also present an implementation on a realistic ARM-based multicore rover platform (running a RT variant of Linux system and realistic security applications). We then perform comparisons with the state-of-the-art~\cite{mhasan_date18} (Section %\ref{sec:evaluation}). 
\ref{sec:exp_rover}).
Finally, we carry out a design space exploration using synthetic workloads and study trade-offs for schedulability and security \hl{(Section} \ref{sec:exp_synthetic}). 
% Key mathematical notations used in the paper are summarized in Table~\ref{tab:mc_math_not}.

\begin{comment}

\begin{table}%[!thb]
% \renewcommand{\arraystretch}{1.3}
\caption{Mathematical Notations}
\label{tab:mc_math_not}
\hspace*{-0.60em}
\centering
%\begin{tabular}{c||p{5.9cm}}
\begin{tabular}{c || P{5.95cm}}
\hline %\\
\bfseries Notation & \bfseries Interpretation\\
\hline\hline
$\Gamma_R$, $\Gamma_S$ & Set of RT and security tasks, respectively \\
$N_R$, $N_S$ & Number of RT and Security tasks, respectively \\
$\mathcal{M}$, $M$ & Set of processor cores and the number of cores, respectively \\
$\pi_m$ & A given processor core \\
$C_i$, $T_i$, $D_i$, $\mathcal{R}_i$ & Worst-case execution time, period, deadline and WCRT of (RT/security) task $\tau_i$, respectively \\
$T_s^{max}$ & Maximum allowable period of security task $\tau_s$ \\
$W_i(x)$ & Workload bound for a job of the task $\tau_i$ within the window of size $x$ \\
% $W_i^{CI}(x)$, $W_i^{NC}(x)$ & Carry-in and non-carry-in workload bound for a window of size $x$ \\
$I_{\tau_j \leftarrow \tau_i}$ & Interference caused by $\tau_i$ on $\tau_j$ \\
% $I_{\tau_j \leftarrow \Gamma_R^{\pi_m}}$ & Total interference on $\tau_j$ from the tasks partitioned on core $\pi_m$ \\
$\Omega_s$ & Total interference experienced by security task $\tau_s$ \\
$hp_S(\tau_s)$, $hp(\tau_s)$ & Set of security tasks and set of all (\ie both RT and security) tasks higher priority than $\tau_s$, respectively \\
$lp(\tau_s)$ & Set of security tasks with a priority lower than $\tau_s$ \\
$\Gamma_s^{CI}$, $\Gamma_s^{NC}$  & Set of carry-in and non-carry-in tasks higher priority than $\tau_s$, respectively \\
$\mathcal{R}_{s | {(\Gamma_s^{NC}, \Gamma_s^{CI}})}$ & Response time of $\tau_s$ for a given carry-in and non-carry-in set \\
\hline
\end{tabular}
\end{table}

\end{comment}

